Categorizing Service Worker Attacks and Mitigations

Service Workers (SWs) are a powerful feature at the core of Progressive Web Apps, namely web applications that can continue to function when the user's device is offline and that have access to device sensors and capabilities previously accessible only by native applications. During the past few years, researchers have found a number of ways in which SWs may be abused to achieve different malicious purposes. For instance, SWs may be abused to build a web-based botnet, launch DDoS attacks, or perform cryptomining; they may be hijacked to create persistent cross-site scripting (XSS) attacks; they may be leveraged in the context of side-channel attacks to compromise users' privacy; or they may be abused for phishing or social engineering attacks using web push notifications-based malvertising. In this paper, we reproduce and analyze known attack vectors related to SWs and explore new abuse paths that have not previously been considered. We systematize the attacks into different categories, and then analyze whether, how, and estimate when these attacks have been published and mitigated by different browser vendors. Then, we discuss a number of open SW security problems that are currently unmitigated, and propose SW behavior monitoring approaches and new browser policies that we believe should be implemented by browsers to further improve SW security. Furthermore, we implement a proof-of-concept version of several policies in the Chromium code base, and also measure the behavior of SWs used by highly popular web applications with respect to these new policies. Our measurements show that it should be feasible to implement and enforce stricter SW security policies without a significant impact on most legitimate production SWs.

==> attack_overview.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Attacks and Abuse of Service Worker's Policies}
\label{sec:attack}
In this section, we discuss new attacks that help circumvent some of the standard policies on service workers as stated in sec\ref{sec:policy_analysis}, thus leading to potential misuse of service workers for malicious purposes. 


\subsection{Stealthy Service Worker}
A major feature of service worker is its capability to run as a background process that can be activated anytime by its owner site by invoking appropriate events such as a {\em Push Event}. Ideally, such invocations to service worker are conveyed to the end-users with the help of visual displays such as {\em Notifications (Custom or Default)}. On receiving the push message, it is a service worker's responsibility to parse the message and display the notification via an API call. Once a service worker is activated it is given a limited period of {XX seconds} to complete data processing and is then put to idle state. Therefore, for an adversary to keep the service worker running, they would have to send multiple push messages constantly before the idle timeout expires. However, this leads to multiple notifications getting displayed from the website which an user might find suspicious and may eventually lead the user to revoke the site's permission to send any notifications.

\begin{lstlisting}[caption={Code Snippet to hide notifications on push event},language=JavaScript, label=code:hide_not_code]
async function hideNotifications()
{
	const notifications = await self.registration.getNotifications();
	for(let i = 0; i < notifications.length; i++) {
	  notifications[i].close();
	  currentNotification.close();
	}
}
self.addEventListener('push', async function (event) {
    event.waitUntil(Promise.all([hideNotifications(),self.registration.showNotification(notification)]));
});
\end{lstlisting}

In this attack, we demonstrate a method to overcome multiple notifications getting displayed to the user and prevent alarming user of any suspicious behavior while keeping the service worker running for a longer duration of time. One of the policies dictate that the API Call \em{showNotification} should be explicitly invoked by a service worker on listening to a push message. Otherwise, a default notification with message {\em 'This site was updated in the background.'} will be displayed. Therefore, in our attack, to prevent the default notification from being shown, we invoke the API \em{registration.showNotification} and immediately invoke a function that parses through the notifications using the API \em{registration.getNotifications} and closes them using the API call \em{Notification.close} as shown in Listing~\ref{code:hide_not_code}. As a result, we are able to activate the service worker and keep it running for a longer duration by repeating the process at frequent intervals. Further, the user is unaware that the service worker is running in the background and an adversary could exploit this feature to perform malicious activities such as DDoS attacks and Cryptomining. As shown in table \ref{tab:hide_not_os}, this attack is effective on multiple operating systems without getting much of user's attention. Further, we demonstrate the feasibility of silent service worker performing DDoS and Cryptomining attacks using a few experiments. For these experiments, we developed a website that registers malicious service workers and we visit the website and grant permission to send notification.  



\input{tables/os_notifications}

\subsubsection{DDoS via Stealthy Service Worker}
In order to perform a DDoS attack, we needed to confirm if an alarming number of requests can be sent by a service worker to any victim server and if there was any restriction on the number of requests posed by the browser. Further, we set up a victim server and the malicious service worker is coded to perform multiple fetch requests to our server, whenever a push event occurs. As a result, we noticed that, on average, the service worker can send up to {\em 50} queries per second to our victim server. Considering this number, an attacker would only require few number of service workers under their control to launch a devastating DDoS attack. We continued this experiment for a duration of 30  minutes and figure~\ref{fig:DDOS_Attack} shows the CPU usage and memory usage by the service worker for the attack duration. During this whole attack, the service worker remained active and hidden without indicating the user of its activities. 


\begin{figure}[!ht]
\centering
\includegraphics[width=\columnwidth]{images/ddos_attack_usage.pdf}
\caption{CPU Usage and Memory Usage by Service Worker involved in DDoS Attack}
\label{fig:DDOS_Attack}
\end{figure}


\subsubsection{CryptoMining via Stealthy Service Worker}
For this experiment, we leverage cryptomining via javascript to illustrate how it can be used to steal computation power from users' machine via hidden service workers. Accordingly, we modify our malicious service worker to invoke the mining script whenever a push event occurs. As a result, we were able to utilize over 100\% of CPU power during the whole duration of the attack. We performed this for over 2.5 hours and found the service worker to be active the whole duration without the user being aware of it. The figure~\ref{fig:Mining_Attack2} shows the the CPU usage and memory usage by the service worker involved in mining Attack.


\begin{figure}[!ht]
\centering
\includegraphics[width=\columnwidth]{images/crypto_mining_attack_usage.pdf}
\caption{CPU Usage and Memory Usage by Service Worker involved in CryptoMining Attack}
\label{fig:Mining_Attack2}
\end{figure}


\subsection{Injecting Malicious Service Workers via Extensions}
Off all restrictions/policies on service workers, the most important is that a service worker can only be registered by a domain if it was served from the same domain. This eliminates the possibility of third parties registering service workers on other domains and preserves the integrity of service workers. In previous studies, it has been shown that attackers could modify the functionality of service workers registered by benign domains by using XSS and redirection attacks. In this attack, we demonstrate how certain features of browser extensions allow them to inject malicious code in any benign domain's service worker. Browser extensions, via certain permissions, have the capability to intercept requests from a web page, monitor them and modify them before the response is sent to the web page. For example, both Google Chrome and Mozilla Firefox browsers allow their extensions to intercept and monitor requests via permissions such as{\em WebRequest} and {\em WebRequestBlocking}. With these permissions, an extension for firefox browser is allowed to use the API, {\em FilterResponse}, that allows extensions to modify the request made for the service worker file at its registration phase. This API is unique to firefox browser and we leverage this functionality to perform this attack. 

\begin{lstlisting}[caption={Code Snippet to modify SW's content from Extension},captionpos=b,language=JavaScript, label=code:ext_code]
function mofifySW(url, reqId) {
	  let filter = browser.webRequest.filterResponseData(reqId);
	  ...
	  filter.ondata = event => {
	      let str = decoder.decode(event.data, {stream: true});
    	  let code_snippet = "self.addEventListener('push', async function (event) {
    	   console.log('Extension:: Received push')} );"
    	  filter.write(encoder.encode(code_snippet+'\n'+str ));
    	  filter.disconnect();
	  }
}
\end{lstlisting}

To test this attack model, we develop a basic extension for firefox that has the capability to intercept requests using {\em WebRequest} and {\em WebRequestBlocking} permissions. Next, we need to filter request that was made for obtaining the service worker script. To achieve this, we use {\em OnBeforeSendHeaders} API to intercept requests and obtain the header information for each requests. By intercepting and analyzing the header information, we filter out Service Worker Script and other scripts that are imported by Service Worker using the header parameter {\em name} assigned to the value {\em Service-Worker}. Then, we read the service worker file's content using the API {\em FilterResponse}. Before sending the file's data, we append a code snippet to the beginning of the file and modify its content. The code snippet that's injected is harmless as shown in Listing~\ref{code:ext_code} as it only adds a listener to {\em Push Event}. In our extension, this listener also sends a dummy request that is used as a way of communicating to the extension that a push event has happened. Accordingly, our extension is designed to alert the user of such a push event via notifications.   



Given the fact that it is not impossible for malicious extensions to be published on official store as discussed in the articles , we believe our attack to be feasible and dangerous if similar approach was adopted by an adversary to publish malicious extension that may only be live for even a shorter duration. Until now, we have known malicious extensions to go unnoticed for over {XX} period of time.  

\input{tables/third_party_libraries}

==> bypass_attack.tex <==
\subsection{Bypass Permission Request}
\label{sec:bypass_attack}
One of the requirements for the previous attack is for the malicious site to obtain user's permission to send notifications. In this section, we demonstrate that it is possible for an adversary to send Web Push Notifications to an end user without requesting for notification permission. This attack is based on the assumption that an attacker already has control of a web page belonging to a benign PWA (Progressive Web Application) by exploiting the vulnerabilities in the site. This attack hinges on the fact that {\em Notification Permission} is granted on an origin level. Therefore, if an attacker controls a page of a benign website that has already been granted permission by the user, attackers can inject their service worker script in the page that they control and start sending push notifications to the user. From the user's perspective, the notifications would be appearing as shown by the benign website. In such a scenario, an user would blindly trust the notifications sent by the adversary and could be easily redirected to pages that may be used to obtain sensitive information from the user. This attack could also be used as a mean to make a website's users lose their trust in the website as they would be getting a lot of annoying or fake notifications. This attack is persistent compared to traditional phishing attacks as even after web pages such as "benign.com/attack" is blocklisted, attacker would still be able to send notifications to the users who have already visited the page once. The only way to end the notifications would be for the user to unregister the service worker of the attacker or revoke notification permission for the entire domain.

\noindent There are two main reasons for this attack to be possible. First, when an user grants permission, it is granted at the domain origin level and domain/website is blindly trusted. Second, any given website can register any number of service workers without user's permission as long as the multiple service workers are registered from different pages of the website. Therefore, we propose that the permission needs to be checked for the domain and service worker. An online demo of this attack is available at this github repository NotificationBypassDemo \footnote{\url{github.com/NotificationBypassDemo/NotificationBypassDemo.github.io}}. 

% the benign PWA as "benign.com" and the web page controlled by attacker as "benign.com/attack" for further explanation. This attack involves the attacker having a service worker script installed on "benign.com/attack" web page that lets attacker to send notifications to user. Consider that "benign.com" already provides WPN service to it's users (refer Figure~\ref{fig:bypassAttack} step 1 ). We also assume that few users exist who have subscribed to WPN service of "benign.com" and granted notification permission. If not, on visitng "benign.com/attack" page an user would be asked for permission as shown in step 2 of Figure~\ref{fig:bypassAttack}. In case of users who have subscribed to WPNs from "benign.com" as shown in step 3 of Figure~\ref{fig:bypassAttack}, if by any means they end up on "benign.com/attack" web page, the attacker's service worker would automatically get registered and the attacker is free to send any number of notifications to the user. Note that the attacker could take advantage of the notification permission already given to "benign.com" and the notifications from attacker would appear to be sent by "benign.com" as shown in step 4 of Figure~\ref{fig:bypassAttack}. In such a scenario, an user would blindly trust the notifications sent by the adversary and could be easily redirected to pages that may be used to obtain sensitive information from the user. This attack could also be used as a mean to make a website's users lose their trust in the website as they would be getting a lot of annoying or fake notifications. This attack is persistent compared to traditional phishing attacks as even after web pages such as "benign.com/attack" is blocklisted, attacker would still be able to send notifications to the users who have already visited the page once. The only way to end the notifications would be for the user to unregister the service worker of the attacker or revoke notification permission for the entire domain.

% \input{tables/bypass_attack_figs.tex}




==> defs.tex <==
\usepackage{xparse}
\newcommand{\bnm}{\begin{newmath}}
\newcommand{\enm}{\end{newmath}}

\newcommand{\bea}{\begin{eqnarray*}}%
\newcommand{\eea}{\end{eqnarray*}}%

\newcommand{\bne}{\begin{newequation}}
\newcommand{\ene}{\end{newequation}}

\newcommand{\bal}{\begin{newalign}}
\newcommand{\eal}{\end{newalign}}

\newenvironment{newalign}{\begin{align}%
\setlength{\abovedisplayskip}{4pt}%
\setlength{\belowdisplayskip}{4pt}%
\setlength{\abovedisplayshortskip}{6pt}%
\setlength{\belowdisplayshortskip}{6pt} }{\end{align}}

\newenvironment{newmath}{\begin{displaymath}%
\setlength{\abovedisplayskip}{4pt}%
\setlength{\belowdisplayskip}{4pt}%
\setlength{\abovedisplayshortskip}{6pt}%
\setlength{\belowdisplayshortskip}{6pt} }{\end{displaymath}}

\newenvironment{neweqnarrays}{\begin{eqnarray*}%
\setlength{\abovedisplayskip}{-4pt}%
\setlength{\belowdisplayskip}{-4pt}%
\setlength{\abovedisplayshortskip}{-4pt}%
\setlength{\belowdisplayshortskip}{-4pt}%
\setlength{\jot}{-0.4in} }{\end{eqnarray*}}

\newenvironment{newequation}{\begin{equation}%
\setlength{\abovedisplayskip}{4pt}%
\setlength{\belowdisplayskip}{4pt}%
\setlength{\abovedisplayshortskip}{6pt}%
\setlength{\belowdisplayshortskip}{6pt} }{\end{equation}}


\newcounter{ctr}
\newcounter{savectr}
\newcounter{ectr}

\newenvironment{newitemize}{%
\begin{list}{\mbox{}\hspace{5pt}$\bullet$\hfill}{\labelwidth=15pt%
\labelsep=4pt \leftmargin=12pt \topsep=3pt%
\setlength{\listparindent}{\saveparindent}%
\setlength{\parsep}{\saveparskip}%
\setlength{\itemsep}{3pt} }}{\end{list}}


\newenvironment{newenum}{%
\begin{list}{{\rm (\arabic{ctr})}\hfill}{\usecounter{ctr} \labelwidth=17pt%
\labelsep=5pt \leftmargin=22pt \topsep=3pt%
\setlength{\listparindent}{\saveparindent}%
\setlength{\parsep}{\saveparskip}%
\setlength{\itemsep}{2pt} }}{\end{list}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
% Figure and table macros
%

\newcounter{mytable}
\def\mytable{\begin{centering}\refstepcounter{mytable}}
\def\endmytable{\end{centering}}

\def\mytablecaption#1{\vspace{2mm}
  \centerline{Table \arabic{mytable}.~{#1}}
  \vspace{6mm}
  \addcontentsline{lot}{table}{\protect\numberline{\arabic{mytable}}~{#1}}
}


\newcounter{myfig}
\def\myfig{\begin{centering}\refstepcounter{myfig}}
\def\endmyfig{\end{centering}}

\def\myfigcaption#1{
             \vspace{2mm}
             \centerline{\textsf{Figure \arabic{myfig}.~{#1}}}
             \vspace{6mm}
             \addcontentsline{lof}{figure}{\protect\numberline{\arabic{myfig}}~{#1}}}


\newlength{\saveparindent}
\setlength{\saveparindent}{\parindent}
\newlength{\saveparskip}
\setlength{\saveparskip}{\parskip}

\newcommand{\decOracle}{\textbf{Dec}}

\newcommand{\negsmidge}{{\hspace{-0.1ex}}}
\newcommand{\cdotsm}{\negsmidge\negsmidge\negsmidge\cdot\negsmidge\negsmidge\negsmidge}

\def\suchthatt{\: :\:}
\newcommand{\E}{{\rm I\kern-.3em E}}
\newcommand{\Prob}[1]{{\Pr\left[\,{#1}\,\right]}}
\newcommand{\Probb}[2]{{\Pr}_{#1}\left[\,{#2}\,\right]}
\newcommand{\CondProb}[2]{{\Pr}\left[\: #1\:\left|\right.\:#2\:\right]}
\newcommand{\CondProbb}[2]{\Pr[#1|#2]}
\newcommand{\ProbExp}[2]{{\Pr}\left[\: #1\:\suchthatt\:#2\:\right]}
\newcommand{\Ex}[1]{{\textnormal{E}\left[\,{#1}\,\right]}}
\newcommand{\Exx}{{\textnormal{E}}}
\newcommand{\given}{\ensuremath{\,\big|\,}}


\newcommand{\true}{\mathsf{true}}
\newcommand{\false}{\mathsf{false}}
\def\negl{\mathsf{negl}}


\newcommand{\secref}[1]{\mbox{Section~\ref{#1}}}
\newcommand{\appref}[1]{\mbox{Appendix~\ref{#1}}}
\newcommand{\thref}[1]{\mbox{Theorem~\ref{#1}}}
\newcommand{\defref}[1]{\mbox{Definition~\ref{#1}}}
\newcommand{\corref}[1]{\mbox{Corollary~\ref{#1}}}
\newcommand{\lemref}[1]{\mbox{Lemma~\ref{#1}}}
\newcommand{\clref}[1]{\mbox{Claim~\ref{#1}}}
\newcommand{\propref}[1]{\mbox{Proposition~\ref{#1}}}
\newcommand{\factref}[1]{\mbox{Fact~\ref{#1}}}
\newcommand{\remref}[1]{\mbox{Remark~\ref{#1}}}
\newcommand{\figref}[1]{\mbox{Figure~\ref{#1}}}
\renewcommand{\algref}[1]{\mbox{Algorithm~\ref{#1}}}
% \newcommand{\eqref}[1]{\mbox{Equation~(\ref{#1})}}
% Have to use \renewcommand because exists already in amsmath
\renewcommand{\eqref}[1]{\mbox{Equation~(\ref{#1})}}
\newcommand{\consref}[1]{\mbox{Construction~\ref{#1}}}
\newcommand{\tabref}[1]{\mbox{Table~\ref{#1}}}

\newcommand{\get}{{\:{\leftarrow}\:}}
\newcommand{\gett}[1]{\:{\leftarrow}_{#1}\:}
\newcommand{\getsr}{{\:{\leftarrow{\hspace*{-3pt}\raisebox{.75pt}{$\scriptscriptstyle\$$}}}\:}}
\newcommand{\getm}{{\:\leftarrow_{\mdist}\:}}
\newcommand{\getd}{{\:\leftarrow_{\ddist}\:}}
%\newcommand{\getm}{{\:{\leftarrow{\hspace*{-3pt}\raisebox{.75pt}{$\scriptscriptstyle \mdist$}}}\:}}
\newcommand{\getk}{{\:\leftarrow_{\kdist}\:}}
%\newcommand{\getk}{{\:{\leftarrow{\hspace*{-3pt}\raisebox{.75pt}{$\scriptscriptstyle \kdist$}}}\:}}
\newcommand{\getp}{{\:\leftarrow_{p}\:}}



\newcommand{\gamesfontsize}{\small}
\newcommand{\fpage}[2]{\framebox{\begin{minipage}[t]{#1\textwidth}\setstretch{1.1}\gamesfontsize  #2 \end{minipage}}}
\newcommand{\mpage}[2]{\begin{minipage}[t]{#1\textwidth}\setstretch{1.1}\gamesfontsize  #2 \end{minipage}}

\newcommand{\hpages}[3]{\begin{tabular}{cc}\begin{minipage}[t]{#1\textwidth} #2 \end{minipage} & \begin{minipage}[t]{#1\textwidth} #3 \end{minipage}\end{tabular}}

\newcommand{\hpagess}[4]{
        \begin{tabular}[t]{c@{\hspace*{.5em}}c}
        \begin{minipage}[t]{#1\textwidth}\gamesfontsize #3 \end{minipage}
        &
        \begin{minipage}[t]{#2\textwidth}\gamesfontsize #4 \end{minipage}
        \end{tabular}
    }

\newcommand{\hpagesss}[6]{
        \begin{tabular}[t]{c@{\hspace*{.5em}}c@{\hspace*{.5em}}c@{\hspace*{.5em}}c}
        \begin{minipage}[t]{#1\textwidth}\gamesfontsize #4 \end{minipage}
        &
        \begin{minipage}[t]{#2\textwidth}\gamesfontsize #5 \end{minipage}
        &
        \begin{minipage}[t]{#3\textwidth}\gamesfontsize #6 \end{minipage}
        \end{tabular}
    }

\newcommand{\hpagessss}[8]{
        \begin{tabular}{c@{\hspace*{.5em}}c@{\hspace*{.5em}}c@{\hspace*{.5em}}c}
        \begin{minipage}[t]{#1\textwidth}\gamesfontsize #5 \end{minipage}
        &
        \begin{minipage}[t]{#2\textwidth}\gamesfontsize #6 \end{minipage}
        &
        \begin{minipage}[t]{#3\textwidth}\gamesfontsize #7 \end{minipage}
        &
        \begin{minipage}[t]{#4\textwidth}\gamesfontsize #8 \end{minipage}
        \end{tabular}
    }


\newcommand{\hfpages}[3]{\hfpagess{#1}{#1}{#2}{#3}}
\newcommand{\hfpagess}[4]{
        \begin{tabular}[t]{c@{\hspace*{.5em}}c}
        \framebox{\begin{minipage}[t]{#1\textwidth}\setstretch{1.1}\gamesfontsize #3 \end{minipage}}
        &
        \framebox{\begin{minipage}[t]{#2\textwidth}\setstretch{1.1}\gamesfontsize #4 \end{minipage}}
        \end{tabular}
    }
\newcommand{\hfpagesss}[6]{
        \begin{tabular}[t]{c@{\hspace*{.5em}}c@{\hspace*{.5em}}c}
        \framebox{\begin{minipage}[t]{#1\textwidth}\setstretch{1.1}\gamesfontsize #4 \end{minipage}}
        &
        \framebox{\begin{minipage}[t]{#2\textwidth}\setstretch{1.1}\gamesfontsize #5 \end{minipage}}
        &
        \framebox{\begin{minipage}[t]{#3\textwidth}\setstretch{1.1}\gamesfontsize #6 \end{minipage}}
        \end{tabular}
    }
\newcommand{\hfpagessss}[8]{
        \begin{tabular}[t]{c@{\hspace*{.5em}}c@{\hspace*{.5em}}c@{\hspace*{.5em}}c}
        \framebox{\begin{minipage}[t]{#1\textwidth}\setstretch{1.1}\gamesfontsize #5 \end{minipage}}
        &
        \framebox{\begin{minipage}[t]{#2\textwidth}\setstretch{1.1}\gamesfontsize #6 \end{minipage}}
        &
        \framebox{\begin{minipage}[t]{#3\textwidth}\setstretch{1.1}\gamesfontsize #7 \end{minipage}}
        &
        \framebox{\begin{minipage}[t]{#4\textwidth}\setstretch{1.1}\gamesfontsize #8 \end{minipage}}
        \end{tabular}
    }

\newcommand{\vecw}{\mathbf{w}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\N}{\mathbb{N}}
\newcommand{\Z}{\mathbb{Z}}
\newcommand{\load}{L}
\newcommand{\coll}{\mathsf{Coll}}
\newcommand{\nocoll}{\overline{\mathsf{Coll}}}


\newcommand{\Img}{\textsf{Img}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%% Fonts and symbols
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand\funcfont{\textsf}
\newcommand\variablefont{\texttt}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% NEW COMMANDS %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\def \Perm {\funcfont{Perm}}
\def \calC {{\mathcal{C}}}
\def \calU {{\mathcal{U}}}
\renewcommand{\u}{\ensuremath{u}}
\newcommand{\unew}{\ensuremath{\tilde{u}}}

\newcommand{\calN}{\mathcal{N}}
\def \sspace {{\mathcal{S}}}
\def \strings {{\mathcal{S}}}
\def \slen {{s}}
\def \kspace {{\mathcal{K}}}
\def \kspacesize {{m}}
\def \mspacesize {{n}}
\def \kdict {D}
\def \dictsize {d}
\newcommand{\kdist}{p_k}
\newcommand{\mdist}{\ensuremath{{W}}}
\newcommand{\alldist}{\rho}
\newcommand{\pwdist}{\transgen}
\newcommand{\ddist}{\rho_{dec}}
\newcommand{\PWset}{{\mathcal{P}}}  % TODO: fix, same as \pwdist
\newcommand{\PWsetvec}{\vec{\mathcal{P}}}
\newcommand{\PWvec}{\vec{P}}
\newcommand{\domvec}{\vec{D}}
\newcommand{\humanornot}{\vec{h}}
\newcommand{\dom}{\textsf{dom}}
%\def \kdist {{\kappa}}
%\def \mdist {{\mu}}
%\def \ddist {{\delta}}
\def \pspace {{\mathcal{P}}}
\def \mpspace {{\mathcal{MP}}}
\def \cspace {{\mathcal{C}}}
\def \key {\kappa}
\def \msg {M}
\def \seed {S}
\def \ctxt {C}
\def \ctxtpart {C_2}
\newcommand{\genprime}{{\textsf{GenPrime}}}
\newcommand{\isprime}{{\textsf{IsPrime}}}
\newcommand{\LeastLesserPrime}{{\textsf{PrevPrime}}}
\newcommand{\pwset}{\mathcal{S}}
\newcommand{\DTE}{{\textsf{DTE}}}
\newcommand{\encode}{{\textsf{encode}}}
\newcommand{\decode}{{\textsf{decode}}}

\newcommand{\DTEsingle}{{\textsf{1PW-DTE}}}
\newcommand{\encodesingle}{{\textsf{1PW-encode}}}
\newcommand{\decodesingle}{{\textsf{1PW-decode}}}

\newcommand{\DTErss}{{\textsf{RSS-DTE}}}
\newcommand{\encoderss}{{\textsf{RSS-encode}}}
\newcommand{\decoderss}{{\textsf{RSS-decode}}}

\newcommand{\DTEindep}{{\textsf{MPW-DTE}}}
\newcommand{\encodeindep}{{\textsf{MPW-encode}}}
\newcommand{\decodeindep}{{\textsf{MPW-decode}}}


\newcommand{\DTEsub}{{\textsf{SG-DTE}}}
\newcommand{\encodesub}{{\textsf{SG-encode}}}
\newcommand{\decodesub}{{\textsf{SG-decode}}}
\newcommand{\decodekamf}{{\textsf{KAMF-decode}}}
\newcommand{\DTEis}{{\textsf{IS-DTE}}}
\newcommand{\encodeis}{{\textsf{is-encode}}}
\newcommand{\decodeis}{{\textsf{is-decode}}}
\newcommand{\DTErej}{{\textsf{REJ-DTE}}}
\newcommand{\encoderej}{{\textsf{rej-encode}}}
\newcommand{\decoderej}{{\textsf{rej-decode}}}
\newcommand{\DTErsarej}{{\textsf{RSA-REJ-DTE}}}
\newcommand{\encodeRSAREJ}{{\textsf{rsa-rej-encode}}}
\newcommand{\decodeRSAREJ}{{\textsf{rsa-rej-decode}}}
\newcommand{\DTErsainc}{{\textsf{RSA-INC-DTE}}}
\newcommand{\encodeRSAINC}{{\textsf{rsa-inc-encode}}}
\newcommand{\decodeRSAINC}{{\textsf{rsa-inc-decode}}}
\newcommand{\DTEunf}{{\textsf{UNF-DTE}}}
\newcommand{\DTEnunf}{{\textsf{NUNF-DTE}}}


%\newcommand{\encodeis}{{\textsf{encode}_{\textrm{is}}}}
%\newcommand{\decodeis}{{\textsf{decode}_{\textrm{is}}}}
\newcommand{\rep}{\textsf{rep}}
\newcommand{\isErr}{\epsilon_{\textnormal{is}}}
\newcommand{\incErr}{\epsilon_{\textnormal{inc}}}
\def \enc {{\textsf{E}}}
\def \dec {{\textsf{D}}}
\def \SEscheme {{\textsf{SE}}}
\def \HEscheme {{\textsf{HE}}}
\def \CTR {{\textsf{CTR}}}
\def \encHE {{\textsf{HEnc}}}
\def \HIDE {{\textsf{HiaL}}}
\def \encHIDE {{\textsf{HEnc}}}
\def \decHIDE {{\textsf{HDec}}}
\def \decHE {{\textsf{HDec}}}
\def \encHEt {{\textsf{HEnc2}}}
\def \decHEt {{\textsf{HDec2}}}

\newcommand{\myind}{\hspace*{1em}}
\newcommand{\thh}{^{\textit{th}}} % th
\newcommand{\concat}{\,\|\,}
\newcommand{\dotdot}{..}
\newcommand{\emptystr}{\varepsilon}

\newcommand{\round}{\textsf{round}}

\newcommand{\alphabar}{\overline{\alpha}}
\newcommand{\numbinsbar}{\overline{b}}
\newcommand{\numballs}{a}
\newcommand{\numbins}{b}

%\def \encHE {{\sf{enc}^{HE}}}
%\def \decHE {{\sf{dec}^{HE}}}
%\def \encHEt {{\sf{enc}^{HE2}}}
%\def \decHEt {{\sf{dec}^{HE2}}}
\def \idealHE {{\mathcal{HE}}}
\def \IEnc {{\mathbf{\rho}}}
\def \IDec {{\mathbf{\rho^{-1}}}}
\def \OEnc {{\mathbf{Enc}}}
\def \ODec {{\mathbf{Dec}}}
\newcommand{\SimuProc}{\mathbf{Sim}}
\newcommand{\ROProc}{\mathbf{RO}}
\newcommand{\PrimProc}{\mathbf{Prim}}
\def \stm {g}
\def \istm {\hat{g}}
\def \kts {{f}}
\def \lex {{\sf lex}}
\def \part {part}
\def \kd {{\sf{kd}}}
\def \msgdist {{d}}
\def \keydist {{r}}
\def \ind {{\sf{index}}}
\def \kprf {z}
\def \adv {{\mathcal A}}
\def \pwds {u}
\newcommand{\mpw}{mpw}
\newcommand{\pw}{w}
\newcommand{\pwvec}{\vec{\pw}}
\newcommand{\vecx}{\vec{x}}
\def \tokens {v}
\def \calP{{\mathcal{P}}}
\def \template{{\mathcal{T}}}
\def \vaultset{{\mathcal{V}}}
\def \ext {{\sf ext}}
\def \offset {\delta}
\def \maxweight {\epsilon}
\def \advo {{\mathcal{A}}^{*}}

\newcommand{\Chall}{\textsf{Ch}}
\newcommand{\Test}{\textnormal{\textsf{Test}}}
\newcommand{\RoR}{\textsf{RoR}}
\newcommand{\MI}{\textnormal{MI}}
\providecommand{\MR}{\textnormal{MR}}
\newcommand{\MRCCA}{\textnormal{MR-CCA}}
\newcommand{\SAMP}{\textnormal{SAMP}}
\newcommand{\DTEgame}{\textnormal{SAMP}}
\newcommand{\KR}{\textnormal{KR}}
\newcommand{\advA}{{\mathcal{A}}}
\newcommand{\advR}{{\mathcal{R}}}
\newcommand{\advB}{{\mathcal{B}}} % 
\newcommand{\advC}{{\mathcal{C}}} % C
\newcommand{\advD}{{\mathcal{D}}} % D
\newcommand{\advE}{{\mathcal{E}}}
\newcommand{\advF}{{\mathcal{F}}}
\newcommand{\advG}{{\mathcal{G}}}
\newcommand{\advI}{{\mathcal{I}}}
\newcommand{\nextval}{\;;\;}
\newcommand{\TabC}{\texttt{C}}
\newcommand{\TabR}{\texttt{R}}
\newcommand{\Hash}{H}
\newcommand{\Cipher}{\pi}
\newcommand{\CipherInv}{\pi^{-1}}
\newcommand{\simu}{{\mathcal S}}
\newcommand{\prim}{P}
\newcommand{\maxguess}{\gamma}


\newcommand{\bigO}{\mathcal{O}}
\newcommand{\calG}{{\mathcal{G}}}

\def\sqed{{\hspace{5pt}\rule[-1pt]{3pt}{9pt}}}
\def\qedsym{\hspace{2pt}\rule[-1pt]{3pt}{9pt}}

\newcommand{\Colon}{{\::\;}}
\newcommand{\good}{\textsf{Good}}

\newcommand\Tvsp{\rule{0pt}{2.6ex}}
\newcommand\Bvsp{\rule[-1.2ex]{0pt}{0pt}}
\newcommand{\TabPad}{\hspace*{5pt}}
\newcommand\TabSep{@{\hspace{5pt}}|@{\hspace{5pt}}}
\newcommand\TabSepLeft{|@{\hspace{5pt}}}
\newcommand\TabSepRight{@{\hspace{5pt}}|}


\DeclareMathOperator*{\argmin}{argmin}
\DeclareMathOperator*{\argmax}{argmax}
\newcommand{\comma}{\textnormal{,}}

\renewcommand{\paragraph}[1]{\vspace*{6pt}\noindent\textbf{#1}\;}

\newcommand{\weirvault}{\textsf{Pastebin}\xspace}
\newcommand{\ndssvault}{\textsf{DBCBW}\xspace}




\newcommand{\reminder}[1]{ [[[ \marginpar{\mbox{$<==$}} #1 ]]] }

%
% New theorem types: (Already in CCS template)
%
\newtheorem{observation}{Observation}
%\newtheorem{definition}{Definition}
\newtheorem{claim}{Claim}
\newtheorem{assumption}{Assumption}
\newtheorem{fact}{Fact}
% \newtheorem{theorem}{Theorem}[section]
% \newtheorem{lemma}{Lemma}[section]
% \newtheorem{corollary}{Corollary}[section]
% \newtheorem{proposition}{Proposition}
% \newtheorem{example}{Example}

%
% Definitions:
%
\def \blackslug{\hbox{\hskip 1pt \vrule width 4pt height 8pt
    depth 1.5pt \hskip 1pt}}
\def \qed{\quad\blackslug\lower 8.5pt\null\par}
% In-line QED, for ending a proof with a $$ formula
% In-line QED, for ending a proof with a $$ formula
\def \inQED{\quad\quad\blackslug}
\def \Qed{\QED}
\def \QUAD{$\Box$}
\def \Proof{\par\noindent{\bf Proof:~}}
\def \proof{\Proof}
\def \poly {\mbox{$\mathsf{poly}$}}
\def \binary {\mbox{$\mathsf{binary}$}}
\def \ones {\mbox{$\mathsf{ones}$}}
\def \rank {\mbox{$\mathsf{rank}$}}
\def \bits {\mbox{$\mathsf{bits}$}}
\def \factorial {\mbox{$\mathsf{factorial}$}}
\def \fr {\mbox{$\mathsf{fr}$}}
\def \pr {\mbox{$\mathsf{pr}$}}
\def \zon {\{0,1\}^n}
\def \zo  {\{0,1\}}
\def \zok {\{0,1\}^k}
\def \mo {s}


\def\utilcnt{\ensuremath{\mu_{\mathrm{cnt}}}}
\def\utiltime{\ensuremath{\mu_{\mathrm{time}}}}
\def\ex{\ensuremath{{\mathrm{ex}}}}
\def\rlx{\ensuremath{{\mathrm{rlx}}}}
\def\tp{\textsf{TP}}
\def\cp{\textnormal{\textsf{CP}}\xspace}
\def\edistcutoff{\edist}
\def\entcutoff{\ensuremath{m}}
\def\relentcutoff{{\sigma}}
\def\mutt{\mu_{\mathrm{tt}}}

\newcommand{\Hdot}{H(\mbox{ } \cdot \mbox{ }  , \mbox{ } \del)}


\newcounter{mynote}[section]
\newcommand{\notecolor}{blue}
\newcommand{\thenote}{\thesection.\arabic{mynote}}
\newcommand{\tnote}[1]{\refstepcounter{mynote}{\bf \textcolor{\notecolor}{$\ll$TomR~\thenote: {\sf #1}$\gg$}}}

\newcommand{\fixme}[1]{{\textcolor{red}{[FIXME: #1]}}}
\newcommand{\todo}[1]{{\textcolor{red}{[TODO: #1]}}}


\newcommand\ignore[1]{}


\newcommand\simplescheme{simple}


\newcommand{\KDF}{\mathsf{KDF}}
\newcommand{\salt}{\mathsf{sa}}
\newcommand{\PRF}{F}
\newcommand{\subgram}{\mathsf{SG}}
\newcommand{\popdomains}{\mathcal{D}}

\newcommand{\retrieve}{\textsf{Sync}}
\newcommand{\update}{\textsf{Insert}}

\newcommand{\dictW}{\textbf{D1}\xspace}
\newcommand{\dictF}{\textbf{D2}\xspace}

\newcommand{\str}{\text{str}}
\newcommand{\calS}{{\mathcal S}}

% \newcommand{\new}[1]{\textcolor{red}{\sf #1}}
\newcommand{\new}[1]{#1}


%% ------------------------- Rahul -----------------------
\newcounter{rcnote}[section]
\newcommand{\rcthenote}{\thesection.\arabic{rcnote}}
\newcommand{\rcnote}[1]{\refstepcounter{rcnote}{\bf \textcolor{magenta}{$\ll$RC~\rcthenote: {\sf #1}$\gg$}}}

\newcounter{mrnote}[section]
\newcommand{\mrthenote}{\thesection.\arabic{mrnote}}
\newcommand{\mrnote}[1]{\refstepcounter{mrnote}{\bf \textcolor{green}{$\ll$MR~\mrthenote: {\sf #1}$\gg$}}}

\newcounter{fknote}[section]
\newcommand{\fkthenote}{\thesection.\arabic{fknote}}
\newcommand{\fknote}[1]{\refstepcounter{fknote}{\bf \textcolor{blue}{$\ll$FK~\fkthenote: {\sf #1}$\gg$}}}

\newcounter{anote}[section]
\newcommand{\ajthenote}{\thesection.\arabic{anote}}
\newcommand{\anote}[1]{\refstepcounter{anote}{\bf \textcolor{cyan}{$\ll$AJ~\ajthenote: {\sf #1}$\gg$}}}



\newcommand{\mytab}{\hspace*{.4cm}}
\def\half{{1\over 2}}
\newcommand{\NT}[1]{\texttt{#1}}
\DeclareMathSymbol{\mlq}{\mathord}{operators}{``}
\DeclareMathSymbol{\mrq}{\mathord}{operators}{`'}
\newcommand{\calO}{{\mathcal O}}
\newcommand{\calA}{{\mathcal A}}
\newcommand{\kamfplus}{Kamouflage\textbf{+}\xspace}
% \newcommand{\genfrom}[1]{\;{\stackrel{\,#1}{\leftarrow}}\;}
\newcommand{\genfrom}[1]{{\:{\leftarrow{\hspace*{-3pt}\raisebox{.75pt}{$\scriptscriptstyle#1$}}}\:}}
%\newcommand{\genfrom}[1]{\;\leftarrow{\tiny \$} #1\;}
\newcommand{\twopartdef}[4]
{
  \left\{
    \begin{array}{ll}
      #1 & \mbox{if } #2 \\[4pt]
      #3 & #4
      \end{array}
      \right.
}
\newcommand{\threepartdef}[6]
{
  \left\{
    \begin{array}{lll}
      #1 & \mbox{if } #2 \\
      #3 & \mbox{if } #4 \\
      #5 & \mbox{if } #6
      \end{array}
      \right.
}

\newcommand{\gt}[1]{\gamma_{#1,\maxdist}}
\newcommand{\gmt}[2]{\gamma_{#1,#2}}
\def\nh{\ensuremath{N}}
\def\ball{\ensuremath{B}}
\def\anh{\ensuremath{\tilde{N}_k}}
% \newcommand{\nh}[2]{{N_{#1}(#2)}}

\newcommand{\ballsizet}[1]{{\beta_{#1,\maxdist}}}
\newcommand{\ballsize}[2]{{\beta_{#1,#2}}}
\newcommand{\rh}[2]{{\bf R}_{#1, #2}}
\newcommand{\rhf}[2]{R_{f, \gamma}}
\newcommand{\realm}{{m}}
% \newcommand{\inputm}{{\tilde{m}}}
\newcommand{\lmid}{\ell_{\realm, m'}}
\newcommand{\cipherlength}{n}
\renewcommand{\SS}{\textsf{SS}}
\newcommand{\Rec}{\textsf{Rec}\xspace}
\newcommand{\rec}{\textsf{rec}\xspace}
\newcommand{\Rep}{\textsf{Rep}\xspace}
\newcommand{\Gen}{\textsf{Gen}}
\newcommand{\dis}{\textsf{dis}}

\def\chk{\textnormal{\textsf{Chk}}\xspace}
\def\reg{\textnormal{\textsf{Reg}}\xspace}
\def\exchk{\textnormal{\textsf{ExChk}}\xspace}
\def\adpchk{\textnormal{\textsf{AdpChk}}\xspace}
\def\RKROR{\textnormal{MKROR}\xspace}
\def\SRKROR{\textnormal{SKROR}\xspace}
\def\ROR{\textnormal{ROR}\xspace}
\def\ROBUST{\textnormal{ROB}\xspace}
\def\OFFDIST{\textnormal{OFFDIST}\xspace}
\def\POFFDIST{\overline{\textnormal{OFFDIST}}\xspace}
\def\OFFGUESS{\textnormal{OFFGUESS}\xspace}
\def\ONGUESS{\overline{\textnormal{ONGUESS}}\xspace}
\def\ONATTACK{\textnormal{ONATTACK}\xspace}
\def\adp{\ensuremath{\Pi\xspace}}
\def\Check{\textnormal{\textsf{Checker}}}
\def\CheckPtxt{\textnormal{\textsf{PChecker}}}
\def\trans{\textnormal{\ensuremath{T}}}
\def\transgen{\textnormal{\ensuremath{\mathcal{T}}}}
\def\pke{\ensuremath{\mathcal{E}}}
\def\pkenc{\ensuremath{\pke^{\mathrm{enc}}}}
\def\pkdec{\ensuremath{\pke^{\mathrm{dec}}}}
\def\sH{\ensuremath\mathrm{H}^s}
\def\H{\ensuremath{\mathsf{H}}\xspace}
\def\T{\ensuremath{\mathsf{T}}\xspace}
\def\W{\ensuremath{\mathsf{W}}\xspace}
\def\F{\ensuremath{\mathsf{F}}\xspace}
\def\ret{\ensuremath{\mathrm{return}}\xspace}
\def\cs{\ensuremath{t}} % Cache Size
\def\waitlen{\ensuremath{\omega}\xspace} %waitlist size
\newcommand{\M}{{\mathcal{M}}}
\newcommand{\ent}{{\bf H}}
\newcommand{\Hfuzzy}{{\mathrm{H}}^{\rm fuzz}}
\newcommand{\Hminfuzzy}{{\mathrm{H}}^{{\rm{fuzz}}}_{t,\infty}}
\newcommand{\Hpfuzzy}{{\mathrm{H}}^{{\rm{pfuzz}}}}
\newcommand{\Hinf}{{\bf H}^{{\rm \min}}_{\infty}}
\newcommand{\Hminpfuzzy}{{\bf H}^{{\rm pfuzz}}_{t,\infty}}


\def\sa{{\sf sa}}
\def\err{{\varepsilon}}%^{(e)}}}
\newcommand{\dist}{\mathcmd{p}}
\newcommand{\distest}{\hat{\mathcmd{p}}}
\newcommand{\distvec}{\mathbf{\dist}}
\newcommand{\distvecest}{\hat{\mathbf{p}}}
\newcommand{\w}{{w}}
\newcommand{\wnew}{\tilde{w}}
\newcommand{\m}{{w}}
\newcommand{\mnew}{{\tilde{m}}}
\newcommand{\mspacevec}{\mathcmd{\mathbf{W}}}
\newcommand{\mvec}{\mathcmd{\mathbf{\m}}}
\newcommand{\mvecss}[1]{\mvec_1\ldots\mvec_{#1}}
\renewcommand{\mspace}{\mathcmd{W}}
\newcommand{\mspacebot}{{\mspace}_\bot}

\newcommand{\similar}{\mathrm{sim}}
\newcommand{\similarvec}{\mathrm{\mathbf{sim}}}

\def \mvecnew{{\tilde{\mvec}}}
\newcommand{\mvecnewss}[1]{\mvecnew_1\ldots\mvecnew_{#1}}

\DeclareDocumentCommand{\edist}{o o}{
  \ensuremath{
    \IfNoValueTF{#1}{{d}}{{\sf d}(#1,#2)}
  }
}

\newcommand{\utilinc}{\mu}
\newcommand{\secloss}{\Delta}
\newcommand{\seclossg}{\Delta^\textnormal{greedy}}
\newcommand{\seclosso}{\Delta}
%\newcommand{\maxlambda}{\lambda^*}
%\newcommand{\maxfuzzlambda}{\tilde{\lambda}^*}
\newcommand{\fuzzlambda}{\lambda^\textnormal{fuzzy}}
\newcommand{\greedylambda}{\lambda^\textnormal{greedy}}
\newcommand{\greedylambdaon}{\tilde{\lambda}^\mathrm{on}}
\newcommand{\greedylambdaoff}{\tilde{\lambda}^\mathrm{off}}
\newcommand{\seclosson}{\secloss^\mathrm{on}}
\newcommand{\seclossoff}{\secloss^\mathrm{off}}
\def \edit {\ensuremath{e}}
\newcommand\error{e}
\newcommand\tab[1][1cm]{\hspace*{#1}}

\newcommand{\mathcmd}[1]{\ensuremath{#1}\xspace} % to use a command both in math mode and non-math mode
\newcommand{\minentropy}[1]{\ensuremath{\operatorname{H_\infty}\olrk{#1}}}
\newcommand{\fuzzyminentropy}[1]{\ensuremath{\operatorname{H^{fuzz}_{\maxdist, \infty}}\olrk{#1}}}
\providecommand{\condminentropy}[2]{\ensuremath{\operatorname{\tilde{H}_\infty}\olrk{#1|#2}}}
\newcommand{\s}{\mathcmd{s}}
\newcommand{\typo}{\mathcmd{\tilde{\m}}}
\newcommand{\typoj}[1]{\ensuremath{(\typo_{#1}, j_{#1})}}
\newcommand\typojprime[1]{{(\typo_{#1}, j'_{#1})}}
\renewcommand\contrib[2]{\mathsf{cont}\left[{#1}/{#2}\right]}
\def\typovec{\ensuremath{\{\typo_i\}_{i=1}}}
\def\opttypovec{\ensuremath{\{\typo^*_i\}_{i=1}}}
\def\slotguess{\textsf{SlotGuess}}
\def\typodist{\ensuremath{\tau_\pw}}
\def\cachedtypodist{\ensuremath{{\tilde{\tau}}_{\pw}}}
\def\typodistest{\ensuremath{{\hat{\tau}}_{\pw}}}
\def\incache{T_\pw}
\newcommand{\fuzzylambda}{\ensuremath{\lambda^{\mathrm{fuzzy}}}}
%\newcommand{\errorprob}[2]{\mathcmd{\tau_{#1}({#2})}}
\newcommand{\errordist}{\mathcmd{\tau}}
\newcommand{\famdist}{\mathcmd{\mathcal{W}}}
\def\guessw{\ensuremath{W}}
\newcommand{\precdist}{W}
\newcommand{\entdef}{Z}
\newcommand{\PW}{\mathcmd{\mathcal{W}}}
\newcommand{\cachedom}{\mathcmd{\mathcal{S}}}
\newcommand{\supp}{\mbox{supp}}
\newcommand{\olrk}[1]{\ifx\nursymbol#1\else\!\!\mskip4.5mu plus 0.5mu\left(\mskip0.5mu plus0.5mu #1\mskip1.5mu plus0.5mu \right)\fi}

\newcommand{\errorprob}[1]{\mathcmd{\tau_{#1}}}
\newcommand{\errorpr}[2]{\mathcmd{\errorprob{#1}{(#2)}}}
\newcommand{\Expectation}{\mathop{\mathbb E}}
\newcommand{\hash}[2]{\mathcmd{F(#1, #2)}}
\newcommand{\hashj}[3]{\mathcmd{F_{#3}(#1, #2)}}
\newcommand{\rhh}{\mathcmd{y}}
\newcommand{\x}{\mathcmd{x}}
\newcommand{\range}{\mathcmd{R}}
\newcommand{\lmm}{\mathcmd{l_\w}}
\newcommand{\rmm}{\mathcmd{r_\w}}
\newcommand{\conflict}[2]{\mathcmd{C_{#1, #2}}}
\newcommand{\Probsub}[2]{{\Pr_{#1}\left[\,{#2}\,\right]}}
\newcommand{\Condprobsub}[3]{{\Pr}_{#1}\left[\: #2\:\left|\right.\:#3\:\right]}
\newcommand{\wmid}{l_{\w, \w^\prime}}
\newcommand{\realhash}{\mathcmd{z}}
\newcommand{\collhash}{\mathcmd{z^\prime}}
\newcommand{\floor}[1]{\left \lfloor #1 \right \rfloor }
\newcommand{\ceiling}[1]{\left \lceil #1 \right \rceil }
\newcommand{\interval}{I}
% \newcommand{\p}[2]{p_{#1}(#2)}
\newcommand{\ssketch}{\mathcmd{\mathsf{S}}}
\newcommand{\tsketch}{\mathcmd{\msgsettingsym\mathsf{S}}}
\newcommand{\trivsketch}{\mathcmd{\tsketch_{\emptystr}}}
\newcommand{\WREC}{\mathcmd{\pcnotionstyle{W\pcmathhyphen{}REC}}}
\newcommand{\AREC}{\mathcmd{\pcnotionstyle{A\pcmathhyphen{}REC}}}
\newcommand{\WUTIL}{\mathcmd{\pcnotionstyle{W\pcmathhyphen{}UTIL}}}
\newcommand{\AUTIL}{\mathcmd{\pcnotionstyle{A\pcmathhyphen{}UTIL}}}
\newcommand{\indexset}{I}
\newcommand{\topset}{Z_1^*}
\newcommand{\cachedist}{T}
\newcommand{\pwdis}{R}
\newcommand{\onbudget}{q}
\newcommand{\blacklist}{\textsf{B}}
\newcommand{\blacklistlen}{\alpha}
\newcommand{\plaintextstate}{\bar{\state}}
\newcommand{\typocutoff}{\delta}
\newcommand{\plfuprob}{\ensuremath{\nu}}

\def\ballweight{\ensuremath{e_{\tilde{\tau}}}}
\newcommand{\Adv}{\textnormal{\textsf{Adv}}}
\newcommand{\AdvOFFLINE}[1]{\Adv^{\footnotesize\textnormal{\textrm{offdist}}}_{\footnotesize #1}}
\newcommand{\AdvOFFLINEP}[1]{\Adv^{\overline{\footnotesize\textnormal{\textrm{{offdist}}}}}_{\footnotesize #1}}
\newcommand{\AdvOFFGUESS}[1]{\Adv^{\footnotesize\textnormal{\textrm{offguess}}}_{\footnotesize #1}}
\newcommand{\AdvONGUESS}[1]{\Adv^{{\footnotesize\textnormal{\textrm{onguess}}}}_{\footnotesize #1}}
\newcommand{\AdvONATTACK}[1]{\Adv^{\footnotesize\textnormal{\textrm{onattack}}}_{\footnotesize #1}}
\newcommand{\AdvRKROR}[1]{\Adv^{\footnotesize\textnormal{\textrm{mk-ror}}}_{\footnotesize #1}}
\newcommand{\AdvSRKROR}[1]{\Adv^{\footnotesize\textnormal{\textrm{sk-ror}}}_{\footnotesize #1}}
\newcommand{\AdvROR}[1]{\Adv^{\footnotesize\textnormal{\textrm{ror}}}_{\footnotesize #1}}
\newcommand{\AdvROBUST}[1]{\Adv^{\footnotesize\textnormal{\textrm{rob}}}_{\footnotesize #1}}

\newcommand{\advantage}[3]{\pcnotionstyle{\Adv}^{#1}_{#2}(#3)}
\newcommand{\neighbourhood}[2]{N_{#1}({#2})}
\newcommand{\rhhdist}{Y}
\newcommand{\fullerhash}{z}
\newcommand{\errorball}[2]{{B}^{\errordist}_{#1}(#2)}
\newcommand{\f}{f}
\newcommand{\pwmaxlen}{\ell}
\newcommand{\indexi}{i}
\newcommand{\indexq}{q}
\newcommand{\indexx}{x}
\newcommand{\replace}{\textsf{replace}}
\newcommand{\vecca}{\vecc{a}}
\newcommand{\veccb}{\vecc{b}}
\newcommand{\veccv}{\vecc{v}}
\newcommand{\coins}{r}
\renewcommand{\state}{\ensuremath{\mathsf{s}}}
\newcommand{\win}{\mathsf{win}}
\newcommand{\Chk}{\textsf{Chk}}
\newcommand{\PChk}{\textsf{PChk}}
\newcommand{\indexh}{h}
\newcommand{\randomZ}{Z}
\newcommand{\Cache}{\textnormal{\textsf{Cache}}}
\newcommand{\WarmupCache}{\textnormal{\textsf{WarmupCache}}}
\newcommand{\CacheUpdate}{\textnormal{\textsf{CacheUpdt}}}
\newcommand{\CacheInit}{\textnormal{\textsf{CacheInit}}}
\newcommand{\cachestate}{\ensuremath{\mathtt{S}}\xspace}
\newcommand{\cachestatelen}{\ensuremath{\sigma}\xspace}
\newcommand{\CacheLRU}{\textnormal{\textsf{CacheLRU}}}
\newcommand{\CacheLRUUpdate}{\textnormal{\textsf{UpdateLRU}}}
\newcommand{\CacheLRUInit}{\textnormal{\textsf{InitLRU}}}


\newcommand{\zxcvbn}{\textnormal{\textsf{zxcvbn}}\xspace}
\newcommand{\bad}{\textnormal{\textsf{bad}}}
\newcommand{\wait}{z}
\newcommand{\PKE}{\textnormal{\textsf{PKE}}}
\newcommand{\pkegen}{\mathcal{K}}
\newcommand{\pkeenc}{\mathcal{E}}
\newcommand{\pkedec}{\mathcal{D}}
\newcommand{\pkectxtspace}{\mathcal{C}_{\pkeenc}}
\newcommand{\pk}{{pk}}
\newcommand{\sk}{{sk}}
\newcommand{\PBE}{\textnormal{\textsf{PBE}}}
\newcommand{\utility}{\textsf{Utility}}

\newcommand{\skegen}{\ensuremath{\mathsf{K}}}
\newcommand{\skeenc}{\ensuremath{\mathsf{E}}}
\newcommand{\skedec}{\ensuremath{\mathsf{D}}}
\newcommand{\skectxtspace}{\ensuremath{\mathcal{C}_{\skeenc}}}
\newcommand{\ske}{\textnormal{\textsf{SKE}}}
\newcommand{\SE}{\textnormal{\textsf{SE}}}
\newcommand{\sekg}{\mathcal{K}}
\newcommand{\seenc}{\mathcal{E}}
\newcommand{\sedec}{\mathcal{D}}
\newcommand{\saltlen}{{\ell_{\mathrm{salt}}}}

\newcommand{\skk}{\textnormal{\textsf{k}}}
\newcommand{\cipherske}{{c}}
\newcommand{\cipherpke}{{c}}
\newcommand{\SH}{\textnormal{\textsf{SH}}}
\newcommand{\FH}{\textnormal{\textsf{H}}}
\newcommand{\counter}{\textnormal{\textsf{Count}}}
\newcommand{\indexp}{p}
\newcommand{\ciphertextspace}{\mathcal{C}}
\newcommand{\states}{\mathcal{S}}
\newcommand{\indexr}{r}
\newcommand{\vecc}[1]{\mathbf{#1}}
\newcommand{\sawait}{\overline{\sa}}
\newcommand{\skkwait}{\overline{\skk}}
\newcommand{\hwait}{\overline{\indexh}}
\newcommand{\randomY}{Y}
\newcommand{\indexm}{m}
\newcommand{\hashtable}[1]{H[#1]}
\newcommand{\SHlen}{k_1}
\newcommand{\FHlen}{k_2}
\newcommand{\valid}{\textnormal{\textsf{valid}}}
\newcommand{\skepsilon}{\epsilon_{ske}}
\newcommand{\pkepsilon}{\epsilon_{pke}}
\newcommand{\hybindex}{j}

\newcommand{\DL}{\textnormal{DL}}
\newcommand{\vecb}{\mathbf{b}}
\newcommand{\indicator}{\mathbb{I}}
\newcommand{\cipherspace}{\mathcal{C}}
\newcommand{\pkemsgspace}{\mathcal{M}_\pkeenc}

\newcommand{\pkecipher}{c}
\newcommand{\skecipher}{{c}}
\newcommand{\pkemsg}{m}
\newcommand{\skemsg}{{m}}
\newcommand{\skemsgspace}{ \msgspace_{\skeenc}}
\newcommand{\upperb}{\alpha}

\newcommand{\ffbox}[1]{
   \setlength{\fboxsep}{-1\fboxrule}
   \fbox{\hspace{1.2pt}\strut#1\hspace{1.2pt}}}


\newcommand{\statespace}{S}
\newcommand{\targuess}{\textsf{TarGuess}}
\newcommand{\untarguess}{\textsf{UnTarGuess}}

\newcommand{\accept}{\texttt{accept}}
\newcommand{\reject}{\texttt{reject}}
\newcommand{\threshold}{\ensuremath{\tau}}
\newcommand{\clfthreshold}{\ensuremath{\theta}}
\newcommand{\far}{\ensuremath{\alpha}}
\newcommand{\frr}{\ensuremath{\beta}}
\newcommand{\fpr}{\ensuremath{\nu}}
\newcommand{\fnr}{\ensuremath{\gamma}}
\newcommand{\FPR}{\textrm{FPR}}
\newcommand{\FNR}{\textrm{FNR}}


\newcommand{\matchalgo}{\mathcal{L}}
\newcommand{\matchalgovec}{\mathcal{\mathbf{L}}_\sslen}
\def \score {\theta}
\newcommand{\indexjvec}{\ensuremath{\mathcmd{\mathbf{j}}\xspace}}
\def\k{k}
\newcommand{\add}{\funcfont{Add}}
\newcommand{\accuracy}{\funcfont{Accuracy}}
\def\acc{\delta}
\def \MS {\funcfont{MS}}
\def \MRec {\funcfont{MRec}}
\newcommand \MSt{\MS^{\matchalgo}_\sslen}
\newcommand \MRect{\MRec^{\matchalgo}_\sslen}
\def \nmatches {\ensuremath{l}}
\def \D{D}
\def \Dmod{\tilde{D}}
\def \mlen{n}
\def \sslen{t}
\def \secret{s}
\def \secretvec{\mathbf{s}}
\newcommand{\sketch}{{\funcfont{sketch}}}
\newcommand{\sketchval}{v}
\def \recover{\funcfont{recover}}
\def \verify{\funcfont{verify}}
\def \q{q}
\def\fp{\alpha}
\def\fn{\beta}
\def\tp{\gamma}
\newcommand{\one}{\ensuremath{\mathbbm{1}}}
\newcommand{\seclen}{\ell}
\newcommand{\Overify}{{\mathcal{O}_\funcfont{vrfy}}}
\newcommand{\Omatch}{\mathcal{O}_\funcfont{match}}
\newcommand{\ith}[2]{#1_{#2}}
\newcommand{\jth}[2]{#1^{#2}}
\newcommand{\mspacei}{\ith{\mspace}{i}}
\newcommand{\errori}{\ith{\error}{i}}
\newcommand{\matchalgoi}{\ith{\matchalgo}{i}}
\newcommand{\mvecbar}{\overline{\mvec}}
\newcommand{\mvectilde}{\tilde{\mvec}}
\newcommand{\angbrac}[1]{\ensuremath{\langle #1 \rangle}}
\newcommand{\clf}{\mathcal{C}}
\newcommand{\clft}{\clf_\sslen}
\newcommand{\clfest}{\mathcal{\hat{\clf}}}
\newcommand{\clfq}[1]{{\clf^q_{#1}}}
\newcommand{\nclf}{r}
\newcommand{\oclf}{\omega}
\newcommand{\biosketch}{\funcfont{TenSketch}\xspace}
\newcommand{\tensketch}{\funcfont{TenSketch}\xspace}

\newcommand{\hvec}{\mathbf{h}}
\newcommand{\insertr}{\mathsf{insert{\scriptstyle\$}}}
\newcommand{\dbmsg}{\ensuremath{\mathcal{F}}}
\newcommand{\dbmsgs}{\ensuremath{\{\dbmsg_i\}}}
\newcommand{\dbid}{\mathcal{I}}
\newcommand{\db}{\ensuremath{D}}
% \newcommand{\dbs}{\ensuremath(\dbid,\{\dbmsg_i\})}
\newcommand{\dbs}{\ensuremath(\dbid,\dbmsg)}
\newcommand{\dbsprime}{\ensuremath(\dbid',\dbmsg')}
\newcommand{\dbsize}{N}
\def \dblen{N}
\def\mhat{\hat{\mvec}}
\def\findmatches{\funcfont{\footnotesize FindMatches$^{\matchalgo}$}}
\newcommand{\setss}[1]{\SS^\Delta_{#1}}
\newcommand{\setrec}[1]{\Rec^\Delta_{#1}}
\newcommand{\setsst}{\setss{\sslen}}
\newcommand{\setrect}{\setrec{\sslen}}
\newcommand{\costs}{{c_s}}
\newcommand{\costc}{{c_c}}
\NewDocumentCommand{\indseq}{ O{1} O{r} }{{#1}\ldots {#2}}
\newcommand{\seq}[2]{{{#1}_1,\ldots,{#1}_{#2}}}
\newcommand{\relu}{\funcfont{ReLu}}
\newcommand{\fcrelu}[1]{\funcfont{FC}_{\relu}^{#1}}
\newcommand{\gencliq}{\funcfont{GenTupIncr}}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main"
%%% End:


==> images/mainflow.tex <==
% \section{Diagrammatic view of Multisketch operations}\label{app:mainflow}  

% A user registers with a user id $\u$ and a vector of biometric templates
% $\mvec=\mvecss{\mlen}$. Multisketch uses two databases $\dbid$ and $\dbmsg$\@,
% where $\dbid$ contains user id $\u$ and the corresponding helper data
% $\sketchval$, and $\dbmsg$ contains the random permutation of the templates
% registered so far. Highlighted are the entries corresponding to a user $\u_4$
% with templates $\mvec_4=\mvec_{41}\ldots\mvec_{4\mlen}$.% and helper
%     % data $\sketchval_4$.
\begin{figure}[t]
  \centering
  \begin{tikzpicture}[
    >=stealth,
    node distance=2cm,
    database/.style={
      cylinder,
      cylinder uses custom fill,
      cylinder body fill=black!25!white,
      cylinder end fill=black!25!white,
      shape border rotate=90,
      aspect=0.25,
      minimum width=2em,
      minimum height=2em,
      draw
    },
    func/.style={
      rectangle,
      fill=red!25!white,
      minimum width=1cm,
      minimum height=1em,
      draw
    },
    cell/.style={
      rectangle,
      draw=black!50!white
    }
    ]
    \node (user) at (0, 0) {User};
    \node[func, right of=user, right=-1.1em, above=3em] (msketch) {$\MS$}; 
    \draw[below of=msketch, dashed, anchor=west] (.85,0.55) rectangle (5.9,-1.2); 
    \node[func, below of=msketch, anchor=east, below=1.95cm,fill=red!10!white,dashed] (mrecover) {$\MRec$};
    % \node[database, right of=user, anchor=south, above=1em, right=2cm] (db1) {$\dbid$};
    \matrix (db1) [right of=user, anchor=south, below=2pt, right=-0.1cm, 
    matrix of math nodes,
    column sep = -\pgflinewidth,
    row sep=-\pgflinewidth,
    column 1/.style={nodes={cell}}, 
    column 2/.style={nodes={cell}}, 
    anchor=west] {
      \u_1 & \sketchval_1\\
      \u_2 & \sketchval_2\\
      \u_3 & \sketchval_3\\
      |[draw,fill=blue!20]|\u_4 & |[draw,fill=blue!20]|\sketchval_4\\
    };
    \node[left of=db1, anchor=east,right=1.1cm] {$\dbid$};
    \matrix (db2) [right of=db1, left=25pt, matrix of math nodes,
    column sep = 2\pgflinewidth,
    row sep=-\pgflinewidth,
    column 1/.style={nodes={cell}},
    column 2/.style={nodes={cell}}, 
    column 3/.style={nodes={cell}}, 
    column 4/.style={nodes={cell}}, 
    column 5/.style={nodes={cell}}, 
    anchor=west] {
      \mvec_{21} &\mvec_{12} & |[draw,fill=blue!20]|\mvec_{43} &  & \mvec_{3\mlen} \\
      |[draw,fill=blue!20]|\mvec_{41} &\mvec_{32} & \mvec_{33} & |[draw=white]|\ldots & \mvec_{2\mlen} \\
      \mvec_{11} &|[draw,fill=blue!20]|\mvec_{42} & \mvec_{23} &  & \mvec_{1\mlen} \\
      \mvec_{31} &\mvec_{22} & \mvec_{13} & & |[draw,fill=blue!20]|\mvec_{4\mlen} \\
    };
    \node[left of=db2, left=-4pt] {$\dbmsg$};

    % \node[database,right of=db1] (db2) {$\dbmsg$};
    \node[func,below of=db1,anchor=north,above=8pt,left=8pt] (gu) {GetUser};
    \node[func,right of=gu,anchor=east,right=-5pt] (fm) {FindMatches};
    \node[func,below of=db1,anchor=east,below=2em,right=-3pt] (recover) {Recover};

    \draw[->,blue!50,thick] (user.north) |- node[black,near end,above]{$u, \mvec$} node[black,near end,below,font=\small]{register} 
    (msketch.west);
    \draw[->,blue!50,thick] (msketch) -| node[black,near end, left,right]{$u, \sketchval$} (db1);
    \draw[->,blue!50,thick] (msketch) -| node[black,near end, left,right]{$\mvec$} (db2);

    \draw[->,blue!50,thick] (user.south) |- ++(1,-0.9) node[black,near end,above]{$u, \mvectilde$} node[black,near end,below,font=\small]{login}   -| node[black,left,near end]{$u$}
    (gu.north);
    \draw[->,blue!50,thick] (user.south) |- ++(0,-0.9)  -- ++(3.1,0) |- node[black,near end, above]{$\mvectilde$}
    (fm.west);
    \draw[->,blue!50,thick] (db1.south) |- node[black,near end,above]{} (gu.east);
    \draw[->,blue!50,thick] (db2.south) |- node[black,near end,above]{} (fm.east);
    \draw[->,blue!50,thick] (gu.south) |- node[black,near end,above]{$\sketchval$} (recover.west);
    \draw[->,blue!50,thick] (fm.south) |- node[black,near end,above]{$\mvec'$} (recover.east);    
    \draw[->,blue!50,line width=2pt] (recover.south) -- node[black,near end,right]{$\mvec$ or $\bot$} ++(0, -0.65);
  \end{tikzpicture}
  % \rcnote{Rough sketch of the flow of the \biosketch.} 
  \caption{Diagram of multisketch as a part of an authentication service. 
  }
  \label{fig:mainflow}
\end{figure}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../main"
%%% End:


==> measurement.tex <==
\section{Measuring Real-World Policies}
\label{sec:measurements}

As mentioned in sec~\ref{sec:overview}, we begin by identifying PWAs in the top 100K Alexa sites. Accordingly, we were able to identify over {XX} PWAs. Then, for detailed analysis, we monitored over {XX} PWAs for a duration of 3 days. In this section, we discuss various measurements obtained as the result of analysis as follows.

\subsection{Policy Measurements}

\subsubsection{Service Worker Lifetime}
Service Worker Lifetime(SWLT) refers to the duration for which service worker was running whenever it was activated due to an event. Further, we also calculate the SWLT per day as sum of the duration for which the service worker running for a total period of 24 hours.  


\subsubsection{Push Events Per Duration}
This measurement refers to the number of push events sent by the websites per duration. For our experiment, we consider this duration as an hour and measure the number of push messages sent by sites at intervals of 1 hour. Please refer to fig.~\ref{fig:push_counts} that shows CDF for push events sent by sites belonging to different bands of ranks. Based on this measurement, we set a threshold {XX} push events per 1 hour for the policy {\em policy-name}.


\begin{figure*}[ht]
\begin{center}
 \begin{subfigure}{.45\textwidth}
    \begin{center}
        \includegraphics[width=\linewidth]{images/cdf_push_count.pdf}
        \label{fig:push_counts}
        \caption{push count per hour}
    \end{center}
 \end{subfigure}%
 \begin{subfigure}{.45\textwidth}
    \begin{center}
        \includegraphics[width=\linewidth]{images/cdf_notification_count.pdf}
        \label{fig:notification_counts}
        \caption{notification count per hour}
    \end{center}
 \end{subfigure}\\[2ex]
 
 \begin{subfigure}{.45\textwidth}
    \begin{center}
        \includegraphics[width=\linewidth]{images/cdf_tp_fetch_count.pdf}
        \label{}
        \caption{third party fetch requests count per second}
    \end{center}
 \end{subfigure} %
 \begin{subfigure}{.45\textwidth}
    \begin{center}
        \includegraphics[width=\linewidth]{images/cdf_tp_origin_count.pdf}
        \label{}
        \caption{third party fetch unique origin count per hour}
    \end{center}
 \end{subfigure} \\[2ex]
 
 \begin{subfigure}{.45\textwidth}
    \begin{center}
        \includegraphics[width=\linewidth]{images/cdf_sw_lifetime.pdf}
        \label{}
        \caption{Lifetime of SW per invocation in minutes}
    \end{center}
 \end{subfigure} %
 \begin{subfigure}{.45\textwidth}
    \begin{center}
        \includegraphics[width=\linewidth]{images/cdf_sw_lifetime_per_day.pdf}
        \label{}
        \caption{Lifetime of SW per day in minutes}
    \end{center}
 \end{subfigure} \\[2ex]
 
  \caption{Policy Measurements shown for each event. Each graph displays the CDF of the event per specific duration for various bands of PWAs a) Push Count per hour  b) Notification Count per hour c) Third-party requests per second d) Third-party origins per hour }
  \label{fig:policy_values}
\end{center}
\end{figure*}


\subsubsection{Notification Events Per Duration}
This measurement refers to the number of notifications that were displayed to the users during a specific interval of time. For our experiment, we consider this duration as an hour and measure the number of push messages sent by sites at intervals of 1 hour. Please refer to fig.~\ref{fig:notification_counts} that shows CDF for push events sent by sites belonging to different bands of ranks. Based on this measurement, we set a threshold {XX} push events per 1 hour for the policy {\em policy-name}.


% \begin{figure}[!ht]
% \centering
% \includegraphics[width=\columnwidth]{images/notification_count.pdf}
% \caption{99th Percentile for Notification Count per 1 hour duration for various bands of sites}
% \label{fig:notification_counts}
% \end{figure}


\subsubsection{Third-party Fetch Events Per Duration}
This measurement refers to the number of third-party fetch events sent by the service worker per duration. As seen from the DDoS attack demo, 50 requests can be sent per second. Moreover, from measurements made from top ranking sites, no more than {xx} requests were made to third-party origins. Therefore, we set a threshold {XX} third-party fetch events per {xx duration} for the policy {\em policy-name}. Figure~\ref{fig:fetch_count} shows the number of fetch events made by SW belonging to sites from different bands of ranks.

\subsubsection{Third-party Requests Origin Count}
This measurement refers to the number of third-party origins that a service worker communicated with. Figure~\ref{fig:origin_count} shows this data for sites from different bands of ranks.


\subsubsection{Notification Close Event Delay }
This delay refers to the difference between the time a notification was shown to the user using the API {\em showNotification} and the notification was closed using the API {\em Notification.close}. As shown in the attacks, closing the notification immediately would hide it from the user while keeping the service worker running in the background. Therefore, this measurement helps us prevent such scenarios. Although, we have seen few cases in the real world where the {\em Notification.close} API was called, we found them to be used for legitimate reasons and didn't find any anomalous behavior during our analysis. However, to prevent this from getting abused in the future, we find a delay value of atleast {\em 30 secs} suitable. Any website falling below this threshold would be flagged anomalous.    


\subsubsection{WPN Ads}
This refers to the number of notifications shown by the websites that led to third-party origin sites when they were clicked. For this project, we consider such cases to be Ads that are delivered via Push Notifications and measure the link between such ads and legitimate sites. 

\subsection{Policy Evaluation}
We need to evaluate the effectiveness of our policies in terms of detecting and stopping malicious behaviour of service workers and not interfering with the behaviour of legitimate service workers. Therefore, we approach this by dividing the legitimate sites into a training set and testing set. Both of these sets are composed of sites belonging to each band of ranks and are selected randomly. The information collected from training set during forensics is used to calculate the policies values' and the policies are then tested on the set of sites belonging to testing set. This testing helps us ensure that our policies do not misidentify legitimate sites and hinder their performance. Further, to test if our policies are sufficient to mitigate the attacks, we also them with the attack demo sites that we have developed. We also calculate how much duration is required for \sysname to detect and mitigate the attacks and the performance overhead that's caused due to real-time detection and mitigation of policy violations. 

For legitimate sites, we select around 10\% of the sites from each band to form the testing set. 

\input{tables/percentile}


==> methodology.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{system Overview}
\label{sec:overview}

In this section, we provide a detailed overview of our system \sysname. Using \sysname, we monitor and measure various aspects of PWAs in the real world to gain better understanding of how service workers are used by web applications. Based on these measurements, we then formulate additional policies that would distinguish malicious/suspicious behavior of PWAs from legitimate ones. Overall, \sysname is made of four major stages. First, a forensic stage that collects information related to service workers from real-world PWAs. Second, a policy analysis stage in which we use the information collected in forensic stage to calculate measurements and formulates policies. Third, an anomaly detection stage that essentially performs the policy checks and detects any violation. Finally, a mitigation stage acts as an enforcer and decide if the policy violations should lead to termination of service worker. All of these stages except the analysis stage  are automated and implemented as part of blink engine in chromium browser. These stages are explained in detail as follows

% In order to get detailed measurements and insights on the PWAs, we instrument Chromium browser to automate certain user actions such as {\em notification click} and log necessary details related to service worker in multiple stages.

\begin{figure*}[t]
  \centering
%   \setlength\belowcaptionskip{-0.7\baselineskip}
  \includegraphics[width=1.0\textwidth]{images/sys_overview.pdf}
%   \addtolength{\belowcaptionskip}{-5pt}
  \caption{SWAT System Overview}
  \label{fig:sys_overview}
\end{figure*} \karthika{ToDo: add the figure for system overview}

\subsection{Forensics Stage}
The forensics stage is responsible to obtain fine-grained information on the usage of Service workers in PWAs. We instrument and hook various events in {\em Service Worker Module} of Blink Engine in Chromium to collect information. Chromium serves as a basis for popular browsers such as Google Chrome, Mozilla Firefox and Microsoft Edge. Therefore, it makes our changes easily portable. These hooks send viable information to our Forensics module that's implemented in the core of blink engine. This Forensics module then logs information about service worker and its related events. These logs are then analyzed offline in the next stage to measure the behaviour of PWAs in the wild and generate policies. In order to standardize our policies in a better way, we derive information from top actors in the domain. Accordingly, we identify PWAs from Alexa's top 100,000 sites and visit each of them using {\em Puppeteer} automation tool and our instrumented browser, and monitor them for few days. The functionalities of our forensics module can be summarized as follows 

\begin{itemize}
    \item To record the life-cycle events of the service worker such as {\em install, activate, update, unregister and termination }
    \item To record any permissions that were requested by the service worker such as push notifications and geo-locations. Further, we also automatically grant these permissions to continue monitoring of how these permissions are utilized.
    \item To record information about the requests that are being made from service worker such as domain name and resources that are fetched
    \item To record API calls made by service worker with respect to caching, push  and notifications service
    \item To simulate user interactions that are required to invoke events of the service worker
    % \item To implement the formulated policies that help identify any anomalous behavior of service worker
    \item To measure CPU, memory and network usage by service workers
\end{itemize}

\subsection{Policy Analysis Stage}
\label{sec:policy_analysis}
At this stage, we manually determine the policies that should be enforced to detect misuse of service workers. In practice, there are certain policies that are enforced by browsers to ensure security to web applications that use service workers and end users who subscribe to these web applications. However, these policies can be circumvented and render ineffective under few attacks as demonstrated later in section~\ref{sec:attack}. Therefore, we pose additional policies that would detect misuse of service workers in a wider manner. Firstly, the standard policies pertaining to service workers as stated by \cite{sw_policies} are as follows

\begin{enumerate}
    \item Only secure contexts can register or use Service Workers
    \item the browser requires that the SW registration URL come from the origin itself
    \item Terminate a SW if the SW has been idle for 30 seconds or if an event takes more than 5 minutes to settle
    \item Push notifications will trigger a user-visible notification if the SW does not create one
\end{enumerate}

As mentioned before, we developed attacks that were able to circumvent these policies without raising any alarm to the users or the browsers. For example, our attacks were able to keep the service worker active for duration beyond 5 minutes thus violating policy 3, prevent any visible notification from being shown to the user, violating policy 4 and let malicious actors modify content of service worker, violating policies 1 and 2. Given the growing trend of websites converting to PWAs, as such the consequences of such violations could be devastating. Moreover, there are more functionalities added to service workers which make them a serious threat. Therefore, we propose some of these additional policies to neutralize the threats posed by service worker while retaining its usefulness.  

\begin{enumerate}
    \item Monitor and limit the overall duration for which a service worker lives in the background
    \item Monitor and limit the number of push events sent by a website for a specified duration
    \item Monitor and limit the number of third-party requests that can be made by the service worker that are unrelated to loading a web page
    \item Monitor and limit the number of notifications that can be shown to the user for a specified duration
    \item Ensure that the notification shown to user remains visible until the user interacts with the notification
    \item Ensure that third-parties don't have access to modify service worker's contents
\end{enumerate}

As stated previously, we consider the usage of SW by Alexa's Top 100K sites to serve as baseline for setting threshold to these policies. Therefore, we divide the top Alexa sites into different bands based on their ranking as shown in Table~\ref{tab:alexa_Ranking}. Different bands are given different priorities based on their rankings and are used to determine reasonable policies.   

\input{tables/alexa_bands}


\subsection{Anomaly Detection Stage}
At this stage, our goal is to devise an automated approach to confirm if the PWAs adhere to the defined policies. We design our anomaly detection module to run dynamically at real-time collecting required information at all points of interest and checking if any policy was violated. We implement this {\em sw\_policy} module as part of modules in blink engine of chromium. Any deviation from these policies could pave way for abuse of the services offered by PWAs. Therefore, in our system, if any policies are circumvented, corresponding information is logged and policy violations are tracked at runtime by the {\em sw\_policy} module. Then, based on the severity of policy violation, our mitigation module (discussed in sec~\ref{sec:mitigation_module}) takes necessary action to thwart service worker. The {\em sw\_policy} module implements the following functionalities 


\begin{enumerate}
    \item Check the state of service worker periodically to know if its running beyond the specified duration in the policies
    \item Record the timestamp of push events sent by a PWA and check if its count for the last specified duration has surpassed the policy threshold 
    \item Record the timestamp of push notifications shown by a PWA and check if its count for the last specified duration has surpassed the policy threshold 
    \item Record the timestamp of third-party fetch requests made by SW and check if its count for the last specified duration has surpassed the policy threshold 
    \item Record the timestamp at which notification is shown and closed and check if the duration falls below the mentioned policy threshold
    \item Prevent third-parties from modifying the content of SW
\end{enumerate}


\subsection{Mitigation Stage}
Any anomalies detected in the previous stage is sent to a mitigation module. This module decides how to deal with these anomalies based on their severity. Further, these anomalies are dealt with immediately at runtime as soon as they are detected without much delay. Based on their severity, one of the following mitigation actions are employed. 

\begin{enumerate}
    \item If the severity is low, a corresponding log is made and its threat level is set to low from none. If multiple policies of severity low are violated, then threat level is increased to medium.
    \item If the severity is medium, then we set the threat level to medium. If the threat level is medium, we immediately terminate the service worker from running. But, it still remains registered.
    \item If the severity is high, then we set the threat to high. We also set the threat level to high, if policies of medium severity are violated repeatedly.  Consequently, we terminate the SW and unregister the service worker.  
\end{enumerate}

\subsection{Implementation Details}
This section includes various details regarding changes made to Chromium browser and using Puppeteer, an automation tool developed by Chrome, for site crawling. For our system, we instrument one of the recent stable versions of Chromium, Version 84.0.4147. Further, we build a docker image containing instrumented Chromium, puppeteer to deploy chromium and the required environment. we plan to publish our instrumentation changes, system implementation, attack PoCs and docker image later for public's use. The implementation details with regards to specific entities are as follows.  

\noindent
\textbf{PWAs and Permissions:}
We consider the sites that register service worker as PWAs and we further narrow our focus on sites that request for notification permission. Firstly, a website registers a SW by invoking the {\em navigator.serviceWorker.register } API call which internally maps to {\em registerServiceWorker} method of \texttt{ServiceWorker\-Container} class. Given that some websites may not register service worker unless the user interacts with the site, we inject {\em Gremlins} library using Puppeteer to simulate random user actions on the webpage and allow a duration of 5 minutes for SW registration. Then, we record the permission request by hooking {\em requestPermission} method of \texttt{NotificationManager} class. In order to grant notification permission, we use puppeteer's API {\em BrowserContext.overridePermissions}. 

\noindent
\textbf{SW Events:}
If a SW imports a script, then the method {importScripts} of {ServiceWorkerGlobalScope} class gets called. All events related to SW after its registration are implemented in \texttt{ ServiceWorker\-GlobalScope} class. The start of events are represented by the methods {\em DispatchPushEvent, DispatchSyncEvent, DispatchNotificationClickEvent, DispatchNotificationCloseEvent, StartFetchEvent} and at the completion of the events, their corresponding handler methods such as {\em  DidHandlePushEvent, DidHandleSyncEvent, DidHandleNotificationClickEvent, DidHandleNotificationCloseEvent, DidHandleFetchEvent} are called respectively. Whenever an event of service worker is invoked, it activates the service worker thread which we obtain from {\em InitializeOnWorkerThread} method of \texttt{Worker\-Thread} class. After the completion of events, when the service worker is terminated it invokes the {\em PrepareForShutdownOnWorkerThread} method. Further. anytime there is an update found for the service worker, the method {\em NotifyUpdateFound} of \texttt{ServiceWorker\-Registration} is called. In the cases where SW uses fetch API to make requests, we obtain the start and end of this call from the methods {\em Fetch} and {\em DidRecieveResponse} of \texttt{FetchManager} class. Therefore, we modify all these methods to call our logger method that records these method calls along with information about service worker such as scope, script URL and request URL related to import and fetch requests. 

\noindent
\textbf{SW CPU \& Memory Usage: }
We also wanted to measure the CPU and memory usage by service workers to check for alarmingly high usage. To record these usage, we leverage the built-in logic for Chromium Task manager. By adding listeners to the taskmanager events, we obtain access to CPU and memory usage and use our logger to record the usage. However, the task manager needs to remain open for the listener to  receive information. Therefore, we use NodeJS library to automatically open Chromium task manager as soon as the browser is launched.   

\noindent
\textbf{Push Notification Events: }
As explained before, listeners to push and notification events such as click and close are recorded in the {ServiceWorkerGlobalScope} class. In order to collect additional information about a displayed notification and its purpose, we automate user clicking the notification by invoking the {\em Click} method of \texttt{NotificationDelegate} class from {\em Add} method under \texttt{Notification\-UIManagerImpl} class. Further, to ensure that we don't interfere with any service worker actions such as a service worker hiding notification once its displayed, we set a delay of 30 seconds before we click on the notification. Usually, these clicks would lead the user to a new page by using {\em openWindow} API which we hook in the \texttt{ServiceWorkerClient} class. 

\noindent
\textbf{SW Policy Implementation: }
We create separate class \texttt{Service\-WorkerPolicies} to keep track of counts related to various policies for each service workers. Then, each time an event occurs, we invoke the corresponding method to update the count and check if it follows the stated policies. In case of violation, we log the violation and based on the severity, stop the service worker. In the case of service-worker-lifetime-policy, we start a timer whenever the service worker was activated. Further, we attach a callback method to the timer which will be called once the timer runs out. This method checks the state of service worker to see if its still running, in which case, we abort the service worker. The timer is cleared if the service worker was terminated automatically before the timer ran out.    




==> new_structure.tex <==
\section{Introduction}

\section{Service Workers Background}
\begin{itemize}
    \item Installation and Scope
    \item Activation Events
    \item Permissions
    \item Javascript APIs
    \item Security Policies
    \item Extensions
    \item Differences among Browsers
\end{itemize}

\section{Service Worker Abuse}
\begin{itemize}
    \item (Malicious) Advertisement
    \item (Stealthy) Continuous Execution
    \item Hijacking
    \item Side Channels 
\end{itemize}

\section{Existing Mitigations and Open Problems}
\begin{itemize}
    \item Content Security Policies
    \item UI Changes and Impact on Permission Granting
    \item Limiting Execution Time
    \item Preventing Stealthy Execution
    \item Limiting Extension-SW Interactions
    \item Browser Isolation
    \item What are the open problems among the above items?
    \begin{itemize}
        \item New UI may still be affected by social engineering
        \item Notification abuse may not violate any Policies
        \item Least privilege principle is not always followed
    \end{itemize}
\end{itemize}

\section{Reducing SW Privileges}
\begin{itemize}
    \item Limiting notification frequency
    \item Limiting CPU times
    \item Preventing extensions' manipulation of SWs
\end{itemize}









==> results.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Evaluation Result}
\label{sec:eval}


==> tables/bypass_attack_figs.tex <==
\begin{figure}[ht]
\caption{Demo of Bypass Notification Attack }
\begin{center}
\label{fig:bypassAttack}
\begin{tabular}{cc}

 \begin{minipage}{.2\textwidth}
      \includegraphics[width=\linewidth]{images/attack_11.PNG}{1}
    \end{minipage}
 & 
\begin{minipage}{.2\textwidth}
      \includegraphics[width=\linewidth]{images/attack_12.PNG}{2}
    \end{minipage}
 \\
\end{tabular}
      \includegraphics[scale=0.7]{images/attack_13.png}{3}
      \includegraphics[scale=0.7]{images/attack_14.png}{4}
\begin{tabular}{c c}
\hline
\end{tabular}
\end{center}
\end{figure}
 

==> tables/csp_bands.tex <==

\begin{table}[htbp]
% \setlength\belowcaptionskip{-0.2\baselineskip}
% \setlength\abovecaptionskip{0.3\baselineskip}
\caption{Bands of Alexa's top 100K sites}
\centering
\label{tab:csp_bands}
% \scriptsize
\resizebox{\columnwidth}{!}{%

% \begin{tabular}{p{1cm}|p{1.2cm}|p{1.2cm}|p{1cm}|p{1cm}}
\begin{tabular}{c|c|c|c|c|c|c}
\toprule
\hline
\textbf{Bands} & {Band\_1} & {Band\_2} & {Band\_3} & {Band\_4} & {Band\_5} &{Total}

\\

\hline
\begin{tabular}[c]{@{}c@{}} \textbf{\#SWs}\\ \textbf{with CSP}\end{tabular} & {20} & {38} & {14} & {64} & {120} & {256}
 
\\
\hline
\begin{tabular}[c]{@{}c@{}} \textbf{\#SWs}\\ \textbf{with CSP }\\ \textbf{ script-src}\end{tabular} & {9} & {3} & {3} & {9} & {21} & {45}
 
\\
\hline
\bottomrule
\end{tabular}

}
% \vspace{-5mm}
\end{table}

==> tables/import_origins.tex <==
\begin{table}[htbp]

\caption{List of Top 10 Third-Party Domains Imported by SWs }
\centering
\label{tab:third_party_imports}
% \scriptsize

\begin{center}
\resizebox{0.55\columnwidth}{!}{%
  \begin{tabular}{c|c}
        \toprule
        \hline
        \begin{tabular}[c]{@{}c@{}}Third-Party  \\ Domains\end{tabular} & \begin{tabular}[c]{@{}c@{}}\# of unique \\ SW Domains\end{tabular} \\\hline
        api.pushnami.com & 196 \\ \hline
        www.gstatic.com & 140 \\ \hline
        cdn.onesignal.com & 95 \\ \hline
        app.najva.com & 63 \\ \hline
        s3.amazonaws.com & 50 \\ \hline
        cdn.subscribers.com & 40 \\ \hline
        cdn.aimtell.com & 35 \\ \hline
        storage.googleapis.com & 33 \\ \hline
        cdn.izooto.com & 31 \\ \hline
        cdn.p-n.io & 28 \\ \hline
        \bottomrule
\end{tabular}
    }
\end{center}

\end{table}
% \vspace{-10pt}

==> tables/os_notifications.tex <==

\begin{table}[htbp]

\caption{Visual Representation in Multiple Platforms }
\centering
\label{tab:hide_not_os}
\resizebox{\linewidth}{!}{%
\begin{tabular}{p{2cm}|p{3cm}|p{3cm}}
\toprule
\hline
{\textbf{Operating System}} 
 & \textbf{Auto-Hide Capability } & \textbf{Visual Representation} \\
\hline

Windows & yes & No visual cue except for the action center icon change that doesn't attract much attention
\\
\hline
Ubuntu & yes & Notification appears and disappears within a second 
\\
\hline
Android & yes & Absolutely No visual cue 
\\
\hline
\bottomrule
\end{tabular}
}
\vspace{-5mm}
\end{table}

==> tables/proposed_mitigations.tex <==
\begin{table}[htpb]

\caption{Overview of SW Abuse and Proposed Mitigations }
\centering
\label{tab:proposed_mitigation}
\scriptsize
\resizebox{\linewidth}{!}{%

\begin{tabular}{l|l|l|l|l|l|l|l}
\hline
\multicolumn{1}{c|}{\multirow{2}{*}{SW Abuse}} & \multicolumn{7}{c|}{Proposed Mitigations} \\ \cline{2-8} 
\multicolumn{1}{c|}{} & \rotatebox{90}{PushCountPerHour} & \rotatebox{90}{PushCountPerDay} & \rotatebox{90}{Third-PartyFetchCount} & \rotatebox{90}{SWLifetimePerInvocation} & \rotatebox{90}{SWLifetimePerDay} & \rotatebox{90}{Scope Isolation} & \rotatebox{90}{Default  SW CSP} 
\\ \hline
Limiting SW Execution Time &  &  &  & \checkmark & \checkmark &  &  \\ \hline
DDoS Attack & \checkmark  &  & \checkmark &  &  &  &  \\ \hline
Phishing \& Malvertising & \checkmark & \checkmark &  &  &  &  &  \\ \hline
XSS Attack &  &  &  &  &  &\checkmark  & \checkmark \\ \hline
LibraryHijack &  &  &  &  &  & \checkmark &  \\ \hline
\end{tabular}

}
\end{table}

==> tables/third_party_libraries.tex <==
\begin{table}[htbp]

\caption{Count of Sites using Third-Party Push Libraries }
\centering
\label{tab:third_party_lib}
% \resizebox{\columnwidth}{!}{%
\begin{tabular}{c|c}
\toprule
\hline
\begin{tabular}[c]{@{}l@{}}Push \\ Library\end{tabular} & \# of Websites \\\hline
OneSignal & 105212 \\\hline
SendPulse & 24003 \\\hline
Vwo.com & 5102 \\\hline
PushAlert & 20000 \\\hline
Pushnami & 1483 \\\hline
PushEngage & 10000 \\\hline
Aimtell & 15000 \\\hline
Wigzo & 1000 \\\hline
PushAssist & 14000 \\\hline
PushWoosh & 88000 \\\hline
FoxPush & 5000 \\\hline
PushPad & 10000 \\\hline

\bottomrule
\end{tabular}
% }
\end{table}

==> usecase.tex <==
\subsection{Use Cases of SW Abuse}

\subsubsection{Continuous Execution Attack}

As discussed, with this category of attacks the user is unaware that the service worker is running in the background and an adversary could exploit this feature to perform malicious activities such as DDoS attacks and Cryptomining. Both of the discussed papers provide experiments proving that their methods can be possibly used for malicious intent. Similarly, we test our attack methods on different browsers and for different purposes and report the results. As shown in table \ref{tab:hide_not_os}, this attack is effective on multiple operating systems without getting much of user's attention. Further, we demonstrate the feasibility of silent service worker performing DDoS and Cryptomining attacks using a few experiments. For these experiments, we developed a website that registers malicious service workers and we visit the website and grant permission to send notification.  

\input{tables/os_notifications}

\noindent \textbf{DDoS via Stealthy Service Worker}
\label{sec:ddos}
In order to perform a DDoS attack, we needed to confirm if an alarming number of requests can be sent by a service worker to any victim server and if there was any restriction on the number of requests posed by the browser. Further, we set up a victim server and the malicious service worker is coded to perform multiple fetch requests to our server, whenever a push event occurs. As a result, we noticed that, on average, the service worker can send up to {\em 50} queries per second to our victim server. Considering this number, an attacker would only require few number of service workers under their control to launch a devastating DDoS attack. We continued this experiment for a duration of 30  minutes and figure~\ref{fig:DDOS_Attack} shows the CPU usage and memory usage by the service worker for the attack duration. During this whole attack, the service worker remained active and hidden without indicating the user of its activities. 


\begin{figure}[!ht]
\centering
\includegraphics[width=\columnwidth]{images/ddos_attack_usage.pdf}
\caption{CPU Usage and Memory Usage by Service Worker involved in DDoS Attack}
\label{fig:DDOS_Attack}
\end{figure}


\noindent \textbf{CryptoMining via Stealthy Service Worker}
For this experiment, we leverage cryptomining via javascript to illustrate how it can be used to steal computation power from users' machine via hidden service workers. Accordingly, we modify our malicious service worker to invoke the mining script whenever a push event occurs. As a result, we were able to utilize over 100\% of CPU power during the whole duration of the attack. We performed this for over 2.5 hours and found the service worker to be active the whole duration without the user being aware of it. The figure~\ref{fig:Mining_Attack2} shows the the CPU usage and memory usage by the service worker involved in mining Attack.


\begin{figure}[!ht]
\centering
\includegraphics[width=\columnwidth]{images/crypto_mining_attack_usage.pdf}
\caption{CPU Usage and Memory Usage by Service Worker involved in CryptoMining Attack}
\label{fig:Mining_Attack2}
\end{figure}


